Schedule-Robust Online Continual Learning

A continual learning (CL) algorithm learns from a non-stationary data stream. The non-stationarity is modeled by some schedule that determines how data is presented over time. Most current methods make strong assumptions on the schedule and have unpredictable performance when such requirements are not met. A key challenge in CL is thus to design methods robust against arbitrary schedules over the same underlying data, since in real-world scenarios schedules are often unknown and dynamic. In this work, we introduce the notion of schedule-robustness for CL and a novel approach satisfying this desirable property in the challenging online class-incremental setting. We also present a new perspective on CL, as the process of learning a schedule-robust predictor, followed by adapting the predictor using only replay data. Empirically, we demonstrate that our approach outperforms existing methods on CL benchmarks for image classification by a large margin.

==> macros_general.tex <==



%----------------------------------------------------------------
\topmargin     0.0cm
\oddsidemargin -0.1cm %-0.1cm
\textwidth     16.8cm%16.8cm
\headheight    0.0cm
\textheight    22.2cm
\parindent     6mm
\parskip       1pt
\tolerance     1000


%----------------------------------------------------------------




%\declaretheorem[name=Theorem,numberlike=theorem]{thm}

\declaretheorem[name=Theorem,refname=Thm.]{theorem}
\declaretheorem[name=Lemma,sibling=theorem]{lemma}
\declaretheorem[name=Proposition,refname=Prop.,sibling=theorem]{proposition}
\declaretheorem[name=Remark]{remark}
\declaretheorem[name=Corollary,refname=Cor.,sibling=theorem]{corollary}
\declaretheorem[name=Definition,refname=Def.]{definition}
\declaretheorem[name=Conjecture,sibling=theorem]{conjecture}
\declaretheorem[name=Axiom]{axiom}
\declaretheorem[name=Assumption,refname=Asm.]{assumption}




\declaretheorem[name=Example]{example}



\def\sectionautorefname{Sec.}
\def\subsectionautorefname{Sec.}


\definecolor{dgreen}{rgb}{0.00,0.49,0.00}
\definecolor{dblue}{rgb}{0,0.08,0.75}
% \usepackage{hyperref}       % hyperlinks
% \RequirePackage[colorlinks,citecolor=green,urlcolor=blue,linkcolor=blue]{hyperref}
\hypersetup{
    colorlinks = true,
    citecolor=dgreen,
    urlcolor=dblue,
    linkcolor=dblue
}


\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{}{}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}
\crefname{section}{Sec.}{Sec.}
\crefname{theorem}{Thm.}{Thm.}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Cor.}{Cor.}
\crefname{example}{Example}{Examples}
\crefname{remark}{Remark}{Remarks}
\crefname{algorithm}{Alg.}{Algorightms}

\crefname{appendix}{Appendix}{Appendices}
\crefname{subappendix}{Appendix}{Appendices}
\crefname{subsubappendix}{Appendix}{Appendices}







\usepackage{etoolbox}


\AfterEndEnvironment{restatable}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{theorem}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{remark}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{example}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{assumption}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{lemma}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{proof}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{corollary}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{proposition}{\noindent\ignorespacesafterend}
\AfterEndEnvironment{definition}{\noindent\ignorespacesafterend}



%------ Names & Acronyms ---------
% \newcommand{\spmlTitle}{A Structured Prediction Approach for Conditional Meta-Learning}
% \newcommand{\paperTitle}{Few-Shot Classification by Meta Label Learning}

\newcommand{\paperTitle}{The Role of Global Labels in Few-Shot Classification and How to Infer Them}


%Few-Shot Classification by Meta Label Learning
%Reformulating FSL / as global MCC 
%The interplay Understating 
\newcommand{\fslong}{few-shot learning}
\newcommand{\fsl}{FSL}
\newcommand{\spml}{TASML}
\newcommand{\laml}{MeLa}
\newcommand{\spmlong}{Task-adaptive Structured Meta-Learning}
\newcommand{\preTrainFeat}{Pre-trained Features}
\newcommand{\lsmetal}{{\textsc{LS~Meta-Learn}}}
\newcommand{\imgnet}{\textsc{ImageNet}}
\newcommand{\mimg}{\textit{mini}\imgnet{}}
\newcommand{\timg}{\textit{tiered}\imgnet{}}
\newcommand{\cifar}{\textsc{CIFAR-FS}}
\newcommand{\leo}{{LEO}}
\newcommand{\sploss}{{\bigtriangleup}}
%---------------------------------

\newcommand{\queryn}{n_q}
\newcommand{\supportn}{n_s}

\newcommand{\msf}[1]{\mathsf{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}


\newcommand{\R}{{\mathbb{R}}}
\newcommand{\N}{{\mathbb{N}}}


\newcommand{\EE}{\mathbb{E}}
\newcommand{\Lagr}{\mathcal{L}}


\newcommand{\X}{{\mathcal{X}}}
\newcommand{\Y}{{\mathcal{Y}}}
\newcommand{\Z}{{\mathcal{Z}}}
\newcommand{\F}{{\mathcal{F}}}
\newcommand{\D}{{\mathcal{D}}}
\newcommand{\A}{{\mathcal{A}}}


\newcommand{\hh}{{\mathcal{H}}}
\newcommand{\G}{{\mathcal{G}}}

\newcommand{\hs}{{\textrm{HS}}}
\newcommand{\HS}{{\hs}}

\newcommand{\alg}{\textrm{Alg}}
\newcommand{\jointAlg}{T}

\newcommand{\condmetapar}{\tau}
\newcommand{\Condmetapar}{{\mathcal{T}}}
\newcommand{\Q}{\mathcal{Q}}

% \newcommand{\citep}{\cite}


\renewcommand{\paragraph}[1]{\noindent{\bfseries #1.}}

\newcommand{\gstar}{{g^*}}


\newcommand{\eqals}[1]{\begin{align*}#1\end{align*}}

\newcommand{\eqal}[1]{\begin{align}#1\end{align}}

\newcommand{\dtr}{S}
\newcommand{\dval}{Q}
\newcommand{\dm}{D_{\rm global}}
\newcommand{\Tau}{\mathcal{T}}
\newcommand{\embd}{\psi_{\theta}}

\providecommand{\scal}[2]{\left\langle{#1},{#2}\right\rangle}
\providecommand{\norb}[1]{\bigl\|{#1}\bigr\|}
\providecommand{\nor}[1]{\left\|{#1}\right\|}

\newcommand{\ridge}{w}

